Scalable Decision-Focused Learning in Restless Multi-Armed Bandits with Application to Maternal and Child Health

This paper studies restless multi-armed bandit (RMAB) problems with unknown arm transition dynamics but with known correlated arm features. The goal is to learn a model to predict transition dynamics given features, where the Whittle index policy solves the RMAB problems using predicted transitions. However, prior works often learn the model by maximizing the predictive accuracy instead of final RMAB solution quality, causing a mismatch between training and evaluation objectives. To address this shortcoming, we propose a novel approach for decision-focused learning in RMAB that directly trains the predictive model to maximize the Whittle index solution quality. We present three key contributions: (i) we establish differentiability of the Whittle index policy to support decision-focused learning; (ii) we significantly improve the scalability of decision-focused learning approaches in sequential problems, specifically RMAB problems; (iii) we apply our algorithm to a previously collected dataset of maternal and child health to demonstrate its performance. Indeed, our algorithm is the first for decision-focused learning in RMAB that scales to real-world problem sizes.

==> checklist.tex <==

\section*{Checklist}
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please refer to Section~\ref{sec:results} about the discussion of the impact of limited data.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Please refer to Section~\ref{sec:results} about the discussion of the significance in maternal and child care domain.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code will be released upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Please refer to Section~\ref{sec:experiments}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Please refer to Appendix~\ref{sec:computation-infrastructure}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{The data are private}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}{}{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Please refer to Section~\ref{sec:experiments}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Please refer to Section~\ref{sec:experiments}}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> learning-curve.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figure/2-state/01220000mdp2s_test_loss.pdf}
        \caption{Testing predictive loss}
        \label{fig:learning-curve-synth-loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figure/2-state/01220000mdp2s_test_OPE_IS.pdf}
        \caption{Testing IS-based evaluation}
        \label{fig:learning-curve-synth-is}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figure/2-state/01220000mdp2s_test_OPE_SIM.pdf}
        \caption{Testing simulation-based evaluation}
        \label{fig:learning-curve-synth-sim}
    \end{subfigure}
    \caption{Comparison between two-stage and decision-focused in the synthetic 2-state fully observable RMAB problems. Two-stage learning can achieve the best predictive loss, but the performance does not translate to evaluation metrics. In contrast, decision-focused learning directly optimizing the importance sampling-based evaluation can generalize the improvement to the simulation-based evaluation. This suggests that there is a weaker correlation between predictive loss and evaluation metrics, but a stronger correlation within evaluation metrics.}
    \label{fig:learning-curve-synth}
\end{figure*}


==> legacy.tex <==
\section{Legacy}


For example, when $s = 0$, the Whittle index $W_i(0)$ is defined by the $m$ such that:
\begin{align}
    V_{i,m}(0) & = m + \gamma \parameter^{p}_{i}(0,0) V_{i,m}(0) + \gamma \parameter^{p}_{i}(0,1) V_{i,m}(1) \nonumber \\
    & = \gamma \parameter^{a}_{i}(0,0) V_{i,m}(0) + \gamma \parameter^{a}_{i}(0,1) V_{i,m}(1) \label{eqn:whittle_index_condition1} \\
    V_{i,m}(1) &= \max \begin{cases}
    m + 1 + \gamma \parameter^{p}_{i}(1,0) V_{i,m}(0) + \gamma \parameter^{p}_{i}(1,1) V_{i,m}(1) \\
    1 + \gamma \parameter^{a}_{i}(1,0) V_{i,m}(0) + \gamma \parameter^{a}_{i}(1,1) V_{i,m}(1)
    \end{cases} \label{eqn:whittle_index_condition2}
\end{align}

Assuming one of the maximum of Equation~\ref{eqn:whittle_index_condition2} holds, we can express Equation~\ref{eqn:whittle_index_condition1} in matrix form:
\begin{align}
    \begin{bmatrix}
        1 & \gamma \parameter^p_i(0,0) - 1 & \gamma \parameter^p_i(0,1) \\
        0 & \gamma \parameter^a_i(0,0) - 1 & \gamma \parameter^a_i(0,1) \\
        1 & \gamma \parameter^p_i(1,0) & \gamma \parameter^p_i(1,1) - 1
    \end{bmatrix} \begin{bmatrix}
        W_i(0) \\
        V_{i,m}(0) \\
        V_{i,m}(1)
    \end{bmatrix} = \begin{bmatrix}
        0 \\
        0 \\ 
        -1
    \end{bmatrix} \label{eqn:whittle_index_result1}
\end{align}
or 
\begin{align}
    \begin{bmatrix}
        1 & \gamma \parameter^p_i(0,0) - 1 & \gamma \parameter^p_i(0,1) \\
        0 & \gamma \parameter^a_i(0,0) - 1 & \gamma \parameter^a_i(0,1) \\
        0 & \gamma \parameter^a_i(1,0) & \gamma \parameter^a_i(1,1) - 1
    \end{bmatrix} \begin{bmatrix}
        W_i(0) \\
        V_{i,m}(0) \\
        V_{i,m}(1)
    \end{bmatrix} = \begin{bmatrix}
        0 \\
        0 \\ 
        -1
    \end{bmatrix} \label{eqn:whittle_index_result2}
\end{align}

One of them will be the real Whittle index. We can compute both of them and plug the corresponding solution $m = W_i(s)$ into Equation~\ref{eqn:whittle_index_condition2} to verify whether the selection is valid. Similarly, $W_i(1)$ can be derived using the same technique.

This argument implies that either Equation~\ref{eqn:whittle_index_result1} or Equation~\ref{eqn:whittle_index_result2} holds. We can therefore explicitly compute the Whittle index by solving either Equation~\ref{eqn:whittle_index_result1} or Equation~\ref{eqn:whittle_index_result2} directly.

The benefit of expressing Whittle index as solution to Equation~\ref{eqn:whittle_index_condition1} and Equation~\ref{eqn:whittle_index_condition2} using either Equation~\ref{eqn:whittle_index_result1} or Equation~\ref{eqn:whittle_index_result2} is that we can get a closed form expression of Whittle index $W_i(s)$ as a function of $\parameter_i$. This allows us to directly compute the derivative of the Whittle index $W_i(s)$ with respect to the MDP parameters $\parameter_i$ without expressing the corresponding optimization problem and KKT conditions.

==> plan.tex <==
\section*{Project Plan}
\paragraph{Step 1:} Build up an evaluation mechanism for the current two stage model that uses off-policy evaluation: We will keep everything the same from the last ARMMAN paper. However, we will use off-policy evaluation to evaluate the performance of policies, rather than doing a real-world experiment, which is obviously extremely costly in terms of real-world costs of people's time. However, off-policy evaluation may also be costly in terms of compute time. Therefore finding fast techniques for off-policy evaluation might be interesting as well. 

We would imagine that our off-policy evaluation is really excellent in that it mirrors real-world performance. As Sanket pointed out, how confident are we of that? So  we might be able to have some idea of how much off-policy evaluation provides an indication for real-world performance -- is there a confidence bound we can provide of how confident we are of our off-policy result? We have real-world performance data and we have off-policy evaluation data. 

\paragraph{Step 2:} Improve the prediction pipeline by evaluating different clustering methods -- potentially methods that might be more easily differentiable. Evaluate with our off-policy evaluation.

\paragraph{Step 3:} Decision-focused learning evaluated via off-policy to see whether that leads to improved results. It is feasible that we learn that decision-focused learning is not useful in this domain. Hopefully that is not the case, but there is some risk here and that is why we want to be sure that we have some other results along the way. (Of course we could write a paper that has a negative result.)

\paragraph{Step 4:} Assuming Step 3 result is a positive one, test Decision-focused learning in the real world or deploy it in the real-world if we have found some way of being super-confident of our evaluations.

==> stitching.tex <==


\subsection{Trajectory Stitching (for Shresth)}
After applying decomposability, we can treat the outcome of each individual beneficiary as a single trajectory with two states (adhering and non-adhering) and two actions (call and not call). The smaller action and state sets of each individual beneficiary makes trajectory stitching more applicable. Specifically, we can compute an empirical transition probability $P'_i$\footnote{This transition probability denotes the transition from $(s,a)$ to $(s', a')$, which also identifies the next action to take. I might need to use a different term for it to avoid confusion. But in short, this is just to simulate the stitching process to produce more trajectories.} for the $i$-th beneficiary by counting the transitions in the trajectory $\trajectory_i = \{ s_{1,i}, a_{1,i}, r_{1,i}, \cdots, s_{T,i}, a_{T,i}, r_{T,i} \}$ for all $i \in [n]$. Any trajectories induced by the empirical transition probability $P'_i$ are valid trajectories that can be produced by the original trajectory $\trajectory_i$. Therefore, we can combine the importance sampling weights, decomposability, stitching by sampling from empirical transition probability to get an enhanced off-policy policy evaluation:
\begin{align}\label{eqn:OPE-stitching}
    \text{OPT}(\policy) = \mathop{\mathbb{E}}\nolimits_{\trajectory_i \sim P'_i ~\forall i \in [n]} \sum\nolimits_{i=1}^n \left[ V_{\trajectory_i}(\policy) \right]
\end{align}

This is the one that we discussed to separate the randomness from the empirical transition probability and the empirical behavioral policy:
\begin{align}\label{eqn:OPE-stitching}
    \text{OPT}(\policy) = \mathop{\mathbb{E}}\nolimits_{\trajectory \sim P, \policy_b} \left[ \mathop{\mathbb{E}}\nolimits_{\trajectory' \sim P', \policy'_{b}} \sum\nolimits_{i=1}^n \left[ V_{\trajectory'_i}(\policy) \right] \right]
\end{align}
where $P', \policy'_{b} = f(\trajectory)$.

\subsection{Different Importance Sampling Weight}
\begin{align}
    & \Pr(\trajectory'_b \mid \policy_b, P) \nonumber \\ = & \sum\nolimits_{\trajectory_b} \Pr(\trajectory'_b \mid \policy_b, P' = f(\trajectory_b)) \Pr(\trajectory_b \mid \pi_b, P)
\end{align}

\begin{align}
    V(\policy_b) & = \mathop{\mathbf{E}}_{\trajectory_b \sim \policy_b, P} V(\trajectory_b) \\
    & = \sum\nolimits_{\trajectory_b} V(\trajectory_b) \Pr(\trajectory_b \mid \policy_b, P) \\
    & = \sum\nolimits_{\trajectory'_b}
\end{align}

\begin{align}
    \Pr{(\trajectory \mid \policy, P)}
\end{align}

\begin{align}
    V(\policy) = \sum\nolimits_{\trajectory} V(\trajectory) \Pr{(\trajectory \mid \policy, P)} 
\end{align}
